Patch-Based Deep Unsupervised Image Segmentation using Graph Cuts

Unsupervised image segmentation aims at grouping different semantic patterns in an image without the use of human annotation. Similarly, image clustering searches for groupings of images based on their semantic content without supervision. Classically, both problems have captivated researchers as they drew from sound mathematical concepts to produce concrete applications. With the emergence of deep learning, the scientific community turned its attention to complex neural network-based solvers that achieved impressive results in those domains but rarely leveraged the advances made by classical methods. In this work, we propose a patch-based unsupervised image segmentation strategy that bridges advances in unsupervised feature extraction from deep clustering methods with the algorithmic help of classical graph-based methods. We show that a simple convolutional neural network, trained to classify image patches and iteratively regularized using graph cuts, naturally leads to a state-of-the-art fully-convolutional unsupervised pixel-level segmenter. Furthermore, we demonstrate that this is the ideal setting for leveraging the patch-level pairwise features generated by vision transformer models. Our results on real image data demonstrate the effectiveness of our proposed methodology.

==> comparison.tex <==
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
    \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/250087_input.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/250087_gt1.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/250087_gt2.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/250087_grapl.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/250087_dfc.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/250087_doubledip.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/250087_picie.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/250087_segsort.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/250087_wnet.png} \\

    \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/279005_input.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/279005_gt1.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/279005_gt2.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/279005_grapl.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/279005_dfc.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/279005_doubledip.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/279005_picie.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/279005_segsort.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/279005_wnet.png} \\

    \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/183066_input.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/183066_gt1.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/183066_gt2.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/183066_grapl.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/183066_dfc.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/183066_doubledip.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/183066_picie.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/183066_segsort.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/183066_wnet.png} \\

    \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/128035_input.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/128035_gt1.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/128035_gt2.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/128035_grapl.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/128035_dfc.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/128035_doubledip.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/128035_picie.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/128035_segsort.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/128035_wnet.png} \\

    \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/28083_input.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/28083_gt1.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/28083_gt2.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/28083_grapl.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/28083_dfc.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/28083_doubledip.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/28083_picie.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/28083_segsort.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/28083_wnet.png} \\

    \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/103029_input.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/103029_gt1.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/103029_gt2.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/103029_grapl.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/103029_dfc.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/103029_doubledip.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/103029_picie.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/103029_segsort.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/103029_wnet.png} \\

\includegraphics[width=0.108\linewidth, valign=b]{comparison_images/201080_input.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/201080_gt1.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/201080_gt2.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/201080_grapl.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/201080_dfc.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/201080_doubledip.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/201080_picie.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/201080_segsort.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/201080_wnet.png} \\

\includegraphics[width=0.108\linewidth, valign=b]{comparison_images/230063_input.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/230063_gt1.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/230063_gt2.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/230063_grapl.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/230063_dfc.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/230063_doubledip.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/230063_picie.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/230063_segsort.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/230063_wnet.png} \\

\includegraphics[width=0.108\linewidth, valign=b]{comparison_images/97010_input.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/97010_gt1.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/97010_gt2.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/97010_grapl.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/97010_dfc.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/97010_doubledip.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/97010_picie.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/97010_segsort.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/97010_wnet.png} \\

\includegraphics[width=0.108\linewidth, valign=b]{comparison_images/365072_input.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/365072_gt1.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/365072_gt2.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/365072_grapl.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/365072_dfc.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/365072_doubledip.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/365072_picie.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/365072_segsort.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/365072_wnet.png} \\

\includegraphics[width=0.108\linewidth, valign=b]{comparison_images/3063_input.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/3063_gt1.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/3063_gt2.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/3063_grapl.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/3063_dfc.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/3063_doubledip.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/3063_picie.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/3063_segsort.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/3063_wnet.png} \\

\includegraphics[width=0.108\linewidth, valign=b]{comparison_images/8068_input.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/8068_gt1.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/8068_gt2.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/8068_grapl.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/8068_dfc.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/8068_doubledip.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/8068_picie.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/8068_segsort.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/8068_wnet.png} \\

\includegraphics[width=0.108\linewidth, valign=b]{comparison_images/2018_input.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/2018_gt1.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/2018_gt2.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/2018_grapl.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/2018_dfc.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/2018_doubledip.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/2018_picie.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/2018_segsort.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/2018_wnet.png} \\

% \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/145059_input.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/145059_gt1.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/145059_gt2.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/145059_grapl.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/145059_dfc.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/145059_doubledip.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/145059_picie.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/145059_segsort.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/145059_wnet.png} \\

% \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/108004_input.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/108004_gt1.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/108004_gt2.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/108004_grapl.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/108004_dfc.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/108004_doubledip.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/108004_picie.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/108004_segsort.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/108004_wnet.png} \\

% \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/101084_input.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/101084_gt1.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/101084_gt2.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/101084_grapl.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/101084_dfc.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/101084_doubledip.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/101084_picie.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/101084_segsort.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/101084_wnet.png} \\

% \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/23050_input.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/23050_gt1.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/23050_gt2.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/23050_grapl.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/23050_dfc.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/23050_doubledip.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/23050_picie.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/23050_segsort.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/23050_wnet.png} \\

% \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/16004_input.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/16004_gt1.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/16004_gt2.png} \hspace{0.01\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/16004_grapl.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/16004_dfc.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/16004_doubledip.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/16004_picie.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/16004_segsort.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/16004_wnet.png} \\

    % & & & & & & & &\\

    % Input & GT 1 & GT 2 & GraPL & DFC & Double & PiCIE & SegSort & W-Net \\
    
    %  & & & & \cite{kim2020unsupervised} & DIP & \cite{cho2021picie} & \cite{hwang2019segsort} & \cite{xia2017w} \\

    %  & & & & & \cite{gandelsman2019double} & & &
\end{tabular}

==> failure_cases.tex <==
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
    \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/156054_input.jpg} & \hspace{0.015\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/156054_gt1.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/156054_gt2.png} & \hspace{0.015\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/156054_grapl.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/156054_dfc.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/156054_doubledip.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/156054_picie.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/156054_segsort.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/156054_wnet.png} \\

    \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/225022_input.jpg} & \hspace{0.015\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/225022_gt2.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/225022_gt1.png} & \hspace{0.015\linewidth} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/225022_grapl.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/225022_dfc.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/225022_doubledip.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/225022_picie.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/225022_segsort.png} & \includegraphics[width=0.108\linewidth, valign=b]{comparison_images/225022_wnet.png} \\

    Input & & GT 1 & GT2 & & GraPL & DFC \cite{kim2020unsupervised} & D-DIP\cite{gandelsman2019double} & PiCIE \cite{cho2021picie} & SegSort \cite{hwang2019segsort} & W-Net \cite{xia2017w} \\
          
\end{tabular}
